The Impact of Time Series Length and Discretization on Longitudinal Causal Estimation Methods

The use of observational time series data to assess the impact of multi-time point interventions is becoming increasingly common as more health and activity data are collected and digitized via wearables, social media, and electronic health records. Such time series may involve hundreds or thousands of irregularly sampled observations. One common analysis approach is to simplify such time series by first discretizing them into sequences before applying a discrete-time estimation method that adjusts for time-dependent confounding. In certain settings, this discretization results in sequences with many time points; however, the empirical properties of longitudinal causal estimators have not been systematically compared on long sequences. We compare three representative longitudinal causal estimation methods on simulated and real clinical data. Our simulations and analyses assume a Markov structure and that longitudinal treatments/exposures are binary-valued and have at most a single jump point. We identify sources of bias that arise from temporally discretizing the data and provide practical guidance for discretizing data and choosing between methods when working with long sequences. Additionally, we compare these estimators on real electronic health record data, evaluating the impact of early treatment for patients with a life-threatening complication of infection called sepsis.

==> sections/background.tex <==
While longitudinal causal estimation methods have grown in popularity in recent
years, their application has largely been restricted to relatively short
sequences. For example, a recent review and comparison of several popular
longitudinal causal estimation methods compared performance on sequences up to
length six \cite{tran2019double}. One notable exception is in the area of
off-policy evaluation of reinforcement learning (RL) algorithms which reduces to longitudinal causal inference from observational data. RL algorithms are
frequently applied over long time horizons and so it is necessary to have
off-policy evaluation methods that scale to long sequences. 

While off-policy evaluation is frequently done using IPW-based estimators,
recent work has used to doubly-robust estimators in order to reduce the variance
of the IPW estimates. For example, \citet{jiang2015doubly} present one such
doubly-robust estimator, observing that it reduces variance relative to IPW
estimators. \citet{thomas2016data} propose a combination of model-based and
IPW-based estimators where the IPW-based estimator is used to estimate reward
up to some time $t$ and the model-based estimator is used for all rewards after
time $t$ where the combination is tuned to minimize mean squared error. These estimators are different those considered in this paper in that they assume the value function has been estimated during policy learning. Further, it is frequently assumed that the observational policy is known and therefore the consistency of IPW and doubly-robust methods is guaranteed.

% Typically, off-policy evaluation is done using IPW-based methods and variance
% is often a concern as in classical causal inference settings [citation];
% however, two commonly made assumptions alleviate these variance concerns
% somewhat in the RL setting. First, it is common to model the environment as a
% time-homogeneous Markov decision process. This greatly reduces the
% dimensionality of the conditional probability of treatment distribution and
% allows for temporal pooling (see section \ref{sec:variance_reduction} for
% details. Second, in many cases, the true probability of treatment distribution
% is known and doesn't need to be estimated. For example, if a company is
% evaluating an ad placement policy using data from its own system, then the
% policy used to generate the data is known. In this case, IPW estimators are
% guaranteed to be consistent and the only downside to their use is variance. For
% this reason, the choice between IPW-based methods and other methods is framed
% as a bias/variance trade-off.
%Lastly, the estimand in off-policy evaluation is typically cumulative reward
%over some time horizon which allows the estimand to be decomposed into a sum
%over time steps.

% Even under these assumptions, the exponential relationship between variance and
% sequence length in importance sampling methods still presents a problem and
% there has been substantial work trying to reduce this variance. 

Another area where longitudinal causal inference methods have been applied to
longer sequences is in the study and optimization of clinical decision making.
\cite{lim2018forecasting} and \citet{li2020g} apply IPW and joint model-based
estimators to synthetic sequences up to length 60 and 64 respectively.
\cite{sofrygin2019targeted} apply a TMLE-based estimator to health record
sequences up to length 143, finding a similar sequence length/variance
relationship. \citet{soleimani2017treatment} and \citet{schulam2017reliable}
sidestep the sequence length issue by using continuous time trajectories.
Finally, \citet{gottesman2018evaluating} review the application of off-policy
evaluation methods to observational health settings, comparing methods on
clinical sequences up to length 20. They focus on how increasing the time
horizon increases the likelihood of sequential positivity violations, which
heavily impacts estimator variance. In contrast, this work focuses on how
sequence length affects estimator bias/variance holding the number samples
constant.


==> sections/contributions.tex <==
1. Empirical comparison of longitudinal causal inference methods on sequences with many timestamps and evaluation of the effect of sequence resolution on variance and bias for each of these estimators.

2. Empirical comparison of longitudinal causal inference methods on clinical data from 

==> sections/discretization_bias_old.tex <==
As we demonstrated in the previous section, choosing how to discretize one's
data represents a bias/variance trade-off. The specifics of this trade-off will
vary depneding on the application and, in this section, we provide
characterization of the bias caused by discretization in the IR and TMLE
estimators so that practitioners may make this decision in an informed manner.
To simplify results, we will assume that the true data generating process obeys
a Markov property. Then, let $\bar{s}$ be a sub-sequence of $\{1,...,T\}$
representing a coarsening of the original feature/treatment sequence with
length $T_{\bar{s}}$ such that $s_1 = 1$ and $s_{T_s} = T$. Typically,
$\bar{s}$ will consist of evenly spaced indices, however, this need not be the
case in general. We will consider the bias incured when the IR and TMLE
estimators are applied to the data coarsened according to $\bar{s}$. For
parsimony, let $\bar{A}_{\bar{s}} = \{A_{s_t}\}_{t=1}^{T_s}$ with an analogous
definition for $\bar{L}_{\bar{s}}$. Then, when applied to the coarsened data,
the IR and TMLE estimators are, in actuality, estimating the following quantity (see the Appendix for a full derivation)
%
% \begin{align}
% 	\psi &= \sum_{\bar{l}_{\bar{s}}} E[Y \mid \bar{A}_{\bar{s}} = \bar{a}_{\bar{s}}, \bar{L}_{\bar{s}} = \bar{l}_{\bar{s}}] \prod_{t=1}^{T_s} p(l_{s_t} \mid \bar{a}_{\bar{s}_{t-1}}, \bar{l}_{\bar{s}_{t-1}})\\\nonumber
% 	&= \sum_{\bar{l}_{\bar{s}}} E[Y \mid A_{T} = a_{T}, L_{T} = l_{T}] \prod_{t=1}^{T_s} p(l_{s_t} \mid a_{s_{t-1}}, l_{s_{t-1}})
% \end{align}
% %
% where the second equality follows from the Markov assumption.
% Then, we can
% expand this expression using the following observation
%
% \begin{align}
% 	p(l_{s_t} \mid a_{s_{t-1}}, l_{s_{t-1}}) = \sum_{l_{s_{t-1}+1},...,l_{s_{t}-1}}  \sum_{a_{s_{t-1}+1},...,a_{s_{t}-1}} p(l_{s_t} \mid a_{s_t-1}, l_{s_t-1}) \prod_{t'=s_{t-1}+1}^{s_{t-1}} p(l_{t'},a_{t'} \mid a_{t'-1}, l_{t'-1})
% \end{align}
%
% By expanding $p(l_{s_t} \mid a_{s_{t-1}}, l_{s_{t-1}})$, we can rewrite this 
%
\begin{align}
	\label{eq:disc_q}
	\sum_{\bar{l}} \sum_{\bar{a}_{\mathbb{N}_{\leq T} \setminus \bar{s}}} 
	 E[Y \mid A_{T} = a_{T}, L_{T} = l_{T}] \left(\prod_{t=1}^{T} p(l_t \mid a_{t-1},l_{t-1})\right) \left(\prod_{t \in \mathbb{N}_{\leq T} \setminus \bar{s}} p(a_t \mid a_{t-1},l_{t-1})\right)
\end{align}
%
Under our causal identifiability assumptions, this corresponds to the
g-computation formula for a stochastic policy where treatment deterministically
follows $\bar{a}_{\bar{s}}$ at all time points in $\bar{s}$ and follows the
observed stochastic policy at all other time points. Importantly, however,
there are no probability of treatment terms for $\bar{A}_{\bar{s}}$. This means
that this stochastic policy may be incoherent in the sense that it may place
non-zero probability on treatment sequences we know to be impossible. For
example, in our synthetic setting, this stochastic policy may violate the assumption that $\bar{A}$ follows a jump process. Evaluating
causal effects under interventions which are not practically realizable is a
hotly contested practice in the causal inference literature [citation];
however, estimating such a quantity may nevertheless be useful if it
approximates the quantity of interest under an intervention that can occur.

This quantity can be used to more rigorously justify a particular choice of discretization bin width. For example, 

% Conceptualizing this stochastic treatment policy may be somewhat difficult;
% however, we can bound the so-called discretization bias $Q_1 - Q_{s,1}$ a
% conceptually simpler quantity. Specifically, by maximizing and minimizing this
% bias over the distributions $p(a_t \mid a_{t-1},l_{t-1})$ for $t \in
% \mathbb{N}_{\leq T} \setminus s$ we can find the worst case bias. In this case,
% the set of stochastic policies that maximize/minimize this bias is guaranteed
% to contain a deterministic policy [citation] and thus we need only consider the
% space of deterministic treatment policies that is consistent with the policy of
% interest $\bar{a}$ at the time points in $\bar{s}$.
%
% \begin{align}
% 	\label{eq:po_upper_bound}
% 	\max_{d:d(a_{s_t - 1},l_{s_t - 1}) = a_{s_t}} E[Y(\bar{a})] - E[Y(d)]
% \end{align}
%
% While we do not want to compute this bound in practice, we may be able to use
% it to reason about the degree of bias induced by coarsening the sequence.

% For example, suppose that we are interested in expected mortality if a
% treatment is started six hours after admission using one hour time bins.
% Further, suppose we are willing to assume a monotonic relationship between
% treatment timing and mortality wherein a delay in treatment does not decrease
% expected mortality. Then, by Equation \ref{eq:po_upper_bound}, we can say that
% the estimate on the coarsened sequence is upper bounded by the expected
% potential outcome were treatment given at hour six and lower bounded by the
% expected potential outcome were treatment given immediately following hour
% five.

==> sections/todos.tex <==
\begin{enumerate}
    \item Clean up plots
    \item Add comments on censoring
    \item Add image captions
    \item Expand citations, particularly around continuous time methods
    \item Simulation results
    \begin{itemize}
        \item Move discussion of specific types of bias to discussion section?
        \item Rework discussion of bias induced by overly-coarse discretization to reflect current discretization process
        \item More general equation for discretization bias? This equation depends on the discretization approach, so a general equation may not be much more useful than a worked example.
    \end{itemize}
\end{enumerate}

\section{Conclusions}
\begin{enumerate}
	
    \item Overly coarse discretization decisions may introduce substantial
    bias, even in cases where there is no time-varying confounding and
    particularly when using the IR and TMLE methods. Overly fine discretization
    decisions may result in excess variance and, in the case of IPW, finite
    sample bias due to sequential positivity violations. When available, domain
    knowledge should be used to define a discretization width that is as coarse
    as possible such that decisions made between timesteps have no (or minimal)
    effect on time-varying features between time steps. In the absence of such
    knowledge, continuous time methods should be considered (e.g.
    \cite{schulam2017reliable,soleimani2017treatment}).
	
    \begin{itemize}
        \item Evidence: Supported by synthetic experiments (Figures 1 and 3).
    \end{itemize}
	
    \item The double robustness property of TMLE comes at the cost of increased
    variance in long sequences (relative to IR). Consistent with the
    recommendations in \citet{hernan2010causal}, practitioners should test the
    sensitivity of conclusions to the choice of estimation method.
	
    \begin{itemize}
        \item Evidence: Supported by both synthetic and real data experiments (Figures 1, 3, and 5).
    \end{itemize}
	
    \item NOT CURRENTLY SUPPORTED, BUT OBSERVED IN SYNTH DATA: When the model
    for $Q$ is misspecified, bias of the IR method increases with sequence
    length. This suggests that using flexible model classes (e.g. [cite
    super-learner]) is even more important when working with long time horizons.
	
    \begin{itemize}
		
        \item This would need more experimentation to demonstrate, but is
        something I observed when designing the synthetic data experiments. It
        is not currently reflected in the results since all models are
        correctly specified.
		
    \end{itemize}

\end{enumerate}

\section{Contributions}
\begin{enumerate}
	
    \item A comparison of the impact of discretization and sequence length
    decisions in simulated data on the bias and variance of three popular
    classes of estimators: inverse probability weighting, iterative regression,
    and targeted minimum-loss estimation.
	
    \item A review and empirical comparison of approaches one can use to reduce
    estimation variance in long sequence settings including pooling across
    time, pooling across treatment regimes, and weight clipping.
	
    \item A comparison of the impact discretization decisions and variance
    reduction methods have on these estimators in a real-time clinical decision
    making setting using electronic health record data with decision sequences
    up to length 72. 
	
\end{enumerate}

